A proposal and evaluation of new timbre visualisation methods for audio sample browsers

Searching through vast libraries of sound samples can be a daunting and time-consuming task. Modern audio sample browsers use mappings between acoustic properties and visual attributes to visually differentiate displayed items. There are few studies focused on how well these mappings help users search for a specific sample. We propose new methods for generating textural labels and positioning samples based on perceptual representations of timbre. We perform a series of studies to evaluate the benefits of using shape, color or texture as labels in a known-item search task. We describe the motivation and implementation of the study, and present an in-depth analysis of results. We find that shape significantly improves task performance, while color and texture have little effect. We also compare results between in-person and online participants and propose research directions for further studies.

==> reference.tex <==

\paragraph{Paragraph headings} Use paragraph headings as needed.


\begin{equation}
a^2+b^2=c^2
\end{equation}

% For one-column wide figures use
\begin{figure}
% Use the relevant command to insert your figure file.
% For example, with the graphicx package use
  \includegraphics{example.eps}
% figure caption is below the figure
\caption{Please write your figure caption here}
\label{fig:1}       % Give a unique label
\end{figure}
%
% For two-column wide figures use
\begin{figure*}
% Use the relevant command to insert your figure file.
% For example, with the graphicx package use
  \includegraphics[width=0.75\textwidth]{example.eps}
% figure caption is below the figure
\caption{Please write your figure caption here}
\label{fig:2}       % Give a unique label
\end{figure*}
%
% For tables use
\begin{table}
% table caption is above the table
\caption{Please write your table caption here}
\label{tab:1}       % Give a unique label
% For LaTeX tables use
\begin{tabular}{lll}
\hline\noalign{\smallskip}
first & second & third  \\
\noalign{\smallskip}\hline\noalign{\smallskip}
number & number & number \\
number & number & number \\
\noalign{\smallskip}\hline
\end{tabular}
\end{table}


==> sections/intro_background.tex <==

\section{Introduction}
\label{intro}
Modern sample libraries can contain thousands of recorded or synthesized sound samples. A common paradigm when searching for a sample is to filter the contents of the library based on keywords or categories and then audition the resulting samples one by one.

\subsection{Information visualisation in media browsers for sound sample search}
Several media browsers have been developed to accelerate this process by placing samples produced by query results in a scatterplot visualisation, or a \textit{starfield display} \citep{ahlberg_visual_1995}.
Some implementations allow users to specify what metadata or audio descriptors to use as the axes of the display \citep{font_design_2010, brazil_audio_2003}, while others use dimensionality reduction (DR) methods to project a high-dimensional set of auditory features to a 2D space \citep{frisson_audiometro:_2014, heise_soundtorch:_2008, font_corbera_freesound_2017}. The latter approach provides less meaningful axes, but can produce an effective clustering of similar sounds. This feature based generation of sample coordinates is often augmented by a visual labeling method. These visual labels can help the user to recognize types of sounds or sounds that they have already auditioned. In existing sample browsers, colors are mapped to timbre features \citep{frisson_audiometro:_2014,brazil_audio_2003, font_freesound_2013, font_corbera_freesound_2017}, and shapes are used to either distinguish categorical variables (e.g. instrument type) \citep{brazil_audio_2003} or to visualize time-varying features \citep{frisson_audiometro:_2014, heise_aurally_2009}. 

\subsection{A novel sample browser with textural labels}
We developed a sound sample browser which lets users visually label sounds using textural images.  It uses a pretrained neural network model \citep{li_universal_2017} for artistic style transfer \citep{gatys_image_2016} to synthesize visual labels for all samples in the library based on a reference set of sound-image pairs. Users can simply choose textural images that they wish to associate with certain sounds and the software takes care of the rest. The advantage of using this method is that no explicit mapping between sound descriptors and visual parameters need to be defined. We think this could be an interesting alternative to the current approach of associating specific audio features to shape or color parameters. Our browser also uses dimensionality reduction of timbre features to place samples in the interface.  

\subsection{Research questions}
While we wish to evaluate the design choices of our sample browser, to what degree \textit{any} of these types of visual labels improve sound search is still an open question. We designed our study to address the following questions:

\begin{itemize}
\item Is there a difference between using color, shape or texture as visual labels in an audio sample browser?
\item Does our timbre feature based placement method assist search, and if so, are these visual labels effective when the information provided by placement is removed?
\end{itemize}


This article presents the design of the study as well as methods for generating visual labels and placing musical samples based on their timbre features. We provide in-depth analysis of results from a group of 15 participants who were recruited to perform the study in a controlled environment. We find that the placement method and shape labels improve participant efficiency, but do not significantly improve task completion time. We also compare these results with a second group of 14 participants who performed the study remotely, but find few commonalities between the two groups.


%Each new image is synthesized to match a weighted combination of the reference images based on the timbre similarity of the samples. 

%
% \citep{heise_soundtorch:_2008} performed a user study comparing their SoundTorch browser to a list-based interface. \citep{frisson_audiometro:_2014} performed several user studies with their AudioMetro browser, which mainly compared the effectiveness of different methods of spatial organisation of the sound samples. As part of their master's thesis, \citep{font_design_2010} performed a study which contrasted using acoustic features as axes against using dimensionality reduction.
\color{red}
\section{Related work}
The field of information visualisation provides a rich resource of theory and guidelines for visual label design. Borgo et al \cite{borgo_glyph-based_2012} provide an extensive review of glyph visualisation, a general form of label designed to communicate values visually. Chen and Floridi \cite{chen_analysis_2013} propose a taxonomy for four types different visual channels: geometric channels (e.g. size, shape, orientation), optical channels (e.g. hue, saturation, brightness, texture, blur, motion), topological and relational channels (e.g. position, distance, connection, intersection) and semantic channels (e.g. numbers, text, symbols).

While visualisation theory principles can be applied to arbitrary sources of information, visualisations of sound can benefit from visual metaphors that appeal to intuitive associations we might make between acoustic and visual properties. 

% Studies of cross-modal correspondences provide useful insights for audio interface design as they highlight associations between vision and audition that a large part of the population might intuitively understand.
The following section presents research on cross-modal correspondences between audition and vision pertinent to the visualisation of timbre. In subsequent sections, we summarize relevant work and user studies in audio browsing.
% similar studies in sound sample browsing.
\color{red}
\subsection{Cross-modal correspondences for timbre visualisation}
\label{sound_vis}
% Conceptually, timbre can be compared with tactile or visual texture; we can use timbre to identify what kind of instrument or process produced a sound in a way analogous to how we might touch or visually inspect an object to identify what materials compose it. 
Studies of cross-modal correspondences provide useful insights for audio interface design as they highlight associations between vision and audition that a large part of the population might intuitively understand.
The \textit{kiki-bouba} experiment \citep {wolfgang_kohler_gestalt_1947} is an early study of such correspondences which found that across cultures and ages, most people associate \textit{"bouba"} with rounder shapes and \textit{"kiki"} with pointed shapes. Recently, an investigation of the cross-modal correspondence of timbre and shapes \cite{adeli_audiovisual_2014} came to a similar conclusion with regard to musical timbre. "Softer" timbres were associated with round shapes, while harsh, "brighter" timbres were associated with spiky shapes. The same work also highlighted a tendency to associate the "soft" timbres with blues and greens and "harsh" timbres with reds and yellows. 

Giannakis and Smith \citep{giannakis_comparative_2006} studied correspondences between acoustic descriptors and visual parameters, furthering work begun by Walker  \citep{walker_effects_1987} on associations between pitch, loudness and visual features such as size, position and lightness. With \textit{Sound Mosaics}, they studied associations between timbre and visual texture using synthesized sounds and images containing repeated elements with varying coarseness, distribution, and granularity among other parameters. They found strong associations between granularity and spectral compactness as well as between coarseness and spectral brightness.

Grill and colleagues performed a study highlighting several high-level perceptual qualities of textural sounds 
\citep{grill_identification_2011} and proposed visualisations \citep{Grill2012VisualizationOP} as well as methods for extracting descriptors \citep{grill_constructing_2012} for each perceptual quality. 
% A study of their visualisation method found that their visual design choices corresponded to participants intuitive audiovisual associations.
Color parameters were used to visualise two of their proposed perceptual metrics: height and tonality (measuring whether a sound is more tone-like or noise-like), which are quite similar to the timbral descriptors for brightness and sprectral flatness. Height was mapped to a range of hue and brightness ranging from bright yellow (high) to dark red (low) and saturation was mapped to tonality.

Berthaut et al. \citep{berthaut_combining_2010} as well as Soraghan \cite{soraghan_animating_2014} studied potential correlations between acoustic properties and those of animated 3D objects. The former found a preference for associating the spectral centroid with color lightness and tonality with texture roughness. The latter found that participants preferred to associate attack time with geometrical resolution, spectral centroid with spikiness and visual brightness with the ratio of even to odd harmonics. Both found that a common preference among participants was much less obvious when multiple mappings were in effect.

% Soraghan proposed several methods visualising timbre for coloring waveforms based on timbral properties as well as 

% These insights inform good practices for visualising timbre, but 
When designing a sample browser incorporating timbre visualisation, developers can either decide on implementing a fixed subset of these acoustic to visual mappings or provide options for users to modify the mappings themselves. While providing a potentially more versatile tool, this second option is dependant on users' knowledge and interpretation of acoustic and visual descriptors. This is what drove us to develop our sample browser which provides a simple method for users to associate textures and timbres by selecting pairs of images and samples.

\subsection{Relevant work in audio browsers}
\label{browsers}

Dimensionality reduction (DR) of low- and high-level audio descriptors is a common practice in audio browser research. A concise overview of commonly used DR methods in audio browsers can be found in \citep{Roma2019AdaptiveMO} and \citep{Stober2013IncrementalVO}. \textit{Islands of Music} \cite{Pampalk2002ContentbasedOA} and \textit{MusicMiner} \cite{Mrchen2005DatabionicVO} popularized using the self-organizing map (SOM) DR method to organize music libraries into topographic maps of musical genres based on a large number of extracted low-level and high-level features. As songs are generally associated with visual metadata such as album covers and pictures of the artists, these can be used to visually differentiate and help users recognize specific songs.

% This approach clearly provides an insightful and stimulating environment for exploring music collections and has been iterated upon by several researchers [][][][], but we could not find studies evaluating the usability of this type of visualisation. 

CataRT \cite{schwarz_real-time_2006}, a tool for sound synthesis and performance, shares many design choices with audio browsers. It displays sound grains (very short sound samples) in a starfield display, allowing users to choose audio descriptors to define each axis and grain colors. Various sonic textures are generated by concatenating grains from user-selected regions of the interface. This tool seems to have been influential in the design of recent drum sample browsers and sequencers. \textit{The infinite drum machine} \citep{kyle_mcdonald_infinite_nodate} demonstrated the creative possibilities of visualising t-SNE DR of drum samples in a web-based drum machine, while \textit{XO} \citep{xln_audio_xo_nodate} is an example of a professional tool based on similar principles. Both tools use color and placement to differentiate sample timbre and allow users to select regions of the sample space to associate with specific beats in a rhythm sequence. Sample color is used to visualise the third dimension of the reduced space in \cite{kyle_mcdonald_infinite_nodate}, while \textit{XO} uses sample color to distinguish predicted drum types (e.g. kick, snare, cymbal).

\color{red}
Stober and Nürnberger developed \textit{MusicGalaxy} \citep{Stober2010MusicGalaxyAM}, a music browser proposing an innovative solution to the commonly occurring issue with dimensionality reduction that some similar elements can be projected to different regions of the reduced space. When focusing on a specific song, its nearest neighbours in the high-dimensional feature space are made obvious by increasing their relative size. In subsequent user studies, this method compared favorably to the more common "pan and zoom" method of navigating large collections.

% proposed  solution draws attention to other similar songs by increasing the size of their neighbours determined in the high-dimensional feature space. 

The following section describes the sample browsers that are closest to ours in design that also incorporated user studies in their development.
\color{black}

\subsection{Studies of audio sample browsers}
\label{other_studies}
% There are, to our knowledge, few other studies on using starfield displays for sound sample search. 
\color{red}
% Hoashi et al. \citep{hoashi} developed an music browser interface and study to compare 2D and 3D visualisations (with placement based on user-selected audio descriptors) to a traditional list-based interface. They found that user performance and preference increased with the number of dimensions.
\color{black}

Heise et al.\citep{heise_soundtorch:_2008} developed \textit{SoundTorch}, which uses a SOM to organize environmental sound samples in 2D space. Participants preferred their method to a list-based interface. They later added a visualisation of the temporal envelope as the contour of each element \citep{heise_aurally_2009}, but did not study the effects of this additional visual information on the effectiveness of the tool.
 
Frisson et al. \citep{frisson_audiometro:_2014} developed AudioMetro, which uses t-SNE DR of audio features and a proximity grid to place sound samples in a starfield display. They also use color and shape labels to differentiate samples. They map the timbre descriptor for brightness to the color lightness channel, and the temporal evolution of sharpness to the contour of the visual labels. Their study mainly evaluated the effect of different methods of spatial organisation of the sound samples, and they offer little analysis of the effect of the labels. 
They remark that simply using DR could cause issues where samples would overlap. Their solution involved moving samples to points on a regular grid. We encountered the same problem but implemented a different solution using simulated springs to push samples apart (section \ref{design:coords}).

% They concluded that their proximity grid approach was more effective than directly using coordinates or a simpler grid-based approach.
% Audiometro uses t-SNE dim reduction on audio features. 
% Compared to a naive grid-based layout, 

In their master’s thesis, Font \citep{font_design_2010} visualized the results of queries to the Freesound database using a starfield display. Their study found that participants were most successful at finding sounds when they could choose sound descriptors as axes. This was compared to placement obtained via PCA DR which they found to perform worse than random placement.

None of these studies looked in-depth into the effect of their choices of visual labels, so we made measuring this effect the main objective of our study design. 



==> sections/results.tex <==

\color{red}
\section{Analysis methods}
\label{analysis_methods}

\subsection{Data transformation}
\label{results:transform}
Initial inspection of collected measures (completion times, hovered samples and total mouse cursor distance) showed that distributions were quite heavily right-tailed. After performing Box-Cox transformations \citep{box_analysis_1964} on each set of measures, statistical models produce normally distributed residuals.\footnote{For a linear regression model to be considered appropriate, the distribution of prediction errors (residuals) should resemble a normal distribution \citep{Martin17}.} 
Mean values and confidence intervals are calculated in transformed values and then back-transformed to their original units. Histograms of the collected measures and transformation parameters are included in the supplementary materials (Online Resource 1, section 2). 

% We use the \textit{forecast} R package \citep{hyndman_forecast_manual} to estimate the optimal transform parameters and to perform the forward and inverse transformations. 

\subsection{Statistical models used to determine the effect of task conditions on performance}
\label{results:models}
% We use general linear mixed-effect models from the \textit{lme4} \citep{bates_lmer} and \textit{lmerTest} \citep{kuznetsova_lmertest} R packages. 
We use general linear mixed-effect models as they support the repeated measures that characterize our study design and account for variance between participants. Task conditions (the placement method and label type) are modeled as fixed effects and a unique identifier assigned to each participant is modeled as a random effect. We report estimated marginal (least-squares) means and confidence intervals. Analysis of variance (ANOVA) of fitted models estimates the probability of equal means.

For significance testing in survey responses, we use the Mann-Whitney U test \citep{mann_test_1947} when comparing between two groups and the Kruskal-Wallis one-way analysis of variance \citep{kruskal_use_1952} when comparing more than two groups.
% Estimated marginal (least-squares) means and confidence intervals of fitted models are calculated with the \textit{emmeans} R package \citep{emmeans_lenth}.

% \begin{table*}[h]
%   \caption{Within-subjects variable levels}
%   \label{table:variables}
%   \begin{tabular}{l l l}
%     \toprule
%     %&&Number of&Number of&&\\
%      \textbf{Variable}& \textbf{Levels} &\textbf{Categories} \\
%     \midrule
%     Placement method & 2 &COORDINATES, RANDOM\\
%     Labelling method & 4 &BASELINE, SHAPE, COLOR, TEXTURE\\
%     % Iteration number & 3 & 1, 2, 3\\
%     \bottomrule
% \end{tabular}
% \end{table*}


\subsection{Packages and notebooks}
% We use the \textit{ggplot2} R package \cite{ggplot} to produce our figures. 
We provide R notebooks for reproducing our results in the supplementary materials repository \citep{richan_timbre_2019} and a complete list of R packages used in the supplementary materials document \citep{richan_study_2019}.
\color{black}
% In addition to these automatically collected metrics, participants complete  questionnaires after the $L_C$ and $L_R$ tasks

\section{Results}
\label{results:intro}
We evaluate the effect of labels and our placement method by comparing means of the recorded measures of task performance calculated from our statistical models. We interpret P-values under 0.05 as strong evidence that the difference between means is significant (not due to chance) \citep{wasserstein_asa_2016}.

%  P-values of the models allow us to ascertain whether the differences between means are statistically significant. 
\subsection{Controlled study with qualified participants}
\label{results:b}
We first investigate the effect of the placement method, followed by that of the labels. Finally we present survey responses of interest.
\subsubsection{Effect of placement method}
\label{results:b:placement}
% Table \ref{table:mean_overall} presents the mean values of measures grouped by placement method.

% \begin{table*}[h]
%   \caption{Means of measures grouped by placement method. Bold p-values indicate when the measured difference between placement methods is significant.\newline CI = 95\% confidence interval. Dim. red. = dimensionality reduction.}
%   \label{table:mean_overall}
%   \begin{tabular}{l l l l l l }
%     \toprule
%     %&&Number of&Number of&&\\
%      \textbf{Measure}& \multicolumn{4}{c}{\textbf{Placement}} & \textbf{p-value}\\
%      \cmidrule(r){2-5}
%       & \textbf{Dim. red.} & CI &\textbf{Random} & CI& \\
%     \midrule
%     Time (s) &11.7  & [10.3, 13.4] & 14.0 &[12.3, 16.1]&\textbf{5.4 e-6}\\
%     Hovered samples &13.0& [11.7, 14.4] &15.4& [13.8, 17.1]&\textbf{0.0019}\\
%     %Mouse speed &251.87&265.62&\textbf{0.0043}\\
%     Total distance (pixels) &2674 & [2465, 2906] & 3286 & [3017, 3583]&\textbf{2.2 e-7}\\
%     \bottomrule
% \end{tabular}
% \end{table*}


% We see a significant difference in average task completion times ($\sim$2.2 seconds faster or $\sim$16\% difference) and  a significant difference in the average number of sounds hovered during tasks ($\sim$2.4 less sounds or $\sim$15\% difference).
% We expected participants performing the random task to cover more distance, as the points are more dispersed. This is confirmed by the significant difference in the average mouse travel distance ($\sim$600 less pixels or $\sim$19\% difference). 

% With our dimensionality reduction (DR) placement method, we see a significant improvement in average task completion times ($\sim$2.3 seconds faster) and  a significant improvement in the average number of sounds hovered during tasks ($\sim$2.4 less sounds).
% We expected participants performing the random task to cover more distance, as the points are more dispersed. This is confirmed by the significant difference in the average mouse travel distance ($\sim$600 less pixels). 

Table \ref{table:mean_label_groups} shows the mean measures grouped by placement method and by label type. In figure \ref{fig:group_means} we plot these means with 95\% confidence intervals. 
We observe that for tasks with baseline labels, participants hovered 3 less samples with dimensionality reduction (DR) placement compared to random placement. Tasks with shape labels also show an $\sim$4 sample improvement with DR placement. For color and texture labels, while mean values of samples hovered are lower with DR placement, the difference is not statistically significant.
The differences in time and distance between placement methods are insignificant for basline tasks. For all label types aside from baseline, the distance travelled by the mouse cursor with random placement is approximately 700 to 800 pixels longer than with DR placement. There is also a significant difference in completion times (approximately 3-4 seconds) in tasks with shape and texture labels.


% We observe that only the number of hovered sounds differ significantly between the baseline tasks. The difference in total distance is significant for all label types aside from baseline. Shape and texture completion times are also significantly worse with random placement. 

\begin{table}[ht]
  \caption{Means of measures grouped by placement and labeling methods. Bold p-values indicate when the difference of mean measures between placement methods is significant.\newline DR = placement by dimensionality reduction.}
  \label{table:mean_label_groups}
  \begin{tabular}{l l l l l}
    \toprule
     \textbf{Measure}& \textbf{Label}& \multicolumn{2}{c}{\textbf{Placement}} & \textbf{p-value}\\
     \cmidrule(r){3-4}
      &&\textbf{DR} &\textbf{Random} & \\
    \midrule
    Time (s) &&&&\\
    & Baseline & 12.3 & 12.7 & 0.54\\
    & Shape & 10.7 & 14.3 & \textbf{0.0008}\\
    & Color & 11.6 & 13.7 & 0.051\\
    & Texture & 11.6 & 15.7 &\textbf{0.0005}\\
    Hovered&&&&\\
    samples& Baseline & 14.9 & 17.9 & \textbf{0.04}\\
    & Shape & 8.7 & 12.5 & \textbf{0.004}\\
    & Color & 13.8 & 15.7 & 0.16\\
    & Texture & 13.5 & 15.3 &0.30\\

    Distance &&&&\\
    (pixels)& Baseline & 2807 & 3094 & 0.12\\
    & Shape & 2313 & 3123 & \textbf{0.0005}\\
    & Color & 2765 & 3588 & \textbf{0.002}\\
    & Texture & 2681 & 3403 & \textbf{0.009}\\
    \bottomrule
\end{tabular}
\end{table}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{images/summer_control_double.eps}
  \caption{Means of task measures grouped by label type and positioning. 95\% confidence intervals shown as error bars.}
\label{fig:group_means}
\end{figure}

\subsubsection{Effect of labeling methods}
\label{results:b:label}
We analyse the effect of labelling methods by comparing them to the baseline tasks. Table \ref{table:mean_diff} summarizes the differences between means. Our main takeaway from these results is that with shape labels, participants need to investigate significantly fewer samples before finding the target sound. Compared to their respective baselines, participants visited on average ~6 less samples in tasks with shape labels before finding the target sound.

Times are not significantly changed when adding visual labels, except in the case of texture labels with random placement, where participants took $\sim$3 seconds longer to find the target sound. 


\begin{table}
  \caption{Mean difference of measures for tasks with labels compared to baseline, grouped by placement method. Positive values indicate an improvement. Bold p-values indicate that the measured difference from the baseline is significant.\newline
    $\overline{B}$ = mean of measures with baseline labels \newline
    $\overline{L}$ = mean of measures with shape, color or texture labels \newline DR = placement by dimensionality reduction.
}
  \label{table:mean_diff}
  \begin{tabular}{l l l l l l}
    \toprule
    %&&Number of&Number of&&\\
     \textbf{Measure}&\textbf{Label} & \multicolumn{4}{c}{\textbf{Placement}} \\
     \cmidrule(r){3-6}
      &&\multicolumn{2}{c}{\textbf{DR}}& \multicolumn{2}{c}{\textbf{Random}} \\
      && \textbf{$\overline{B} -\overline{L}$} &\textbf{\textit{p-val.}}&\textbf{$\overline{B} -\overline{L}$}  &\textbf{\textit{p-val.}}\\
    \midrule
    Time (s) &&&&\\
    & Shape   & 1.59 & 0.18 &-1.58 & 0.26\\
    & Color   & 0.76 & 1.0 &-0.9  & 1.0\\
    & Texture & 0.73 & 0.96 &-2.91 & \textbf{0.03} \\
    Hovered&&&&\\
    samples& Shape & 6.1 & \textbf{4e-07} &5.5 & \textbf{0.002}\\
    & Color & 1.1 & 0.89  & 2.3 & 0.52 \\
    & Texture & 1.3 & 0.33  & 2.7 & 0.13 \\
    Distance &&&&\\
    (pixels) & Shape & 494 & \textbf{0.04} & -30 & 1.0 \\
    & Color & 41 & 1.0  & -493 & 0.20 \\
    & Texture & 120 & 0.94  & -307 & 0.61 \\
    
    \bottomrule
\end{tabular}
\end{table}


% \begin{table*}[h]
%   \caption{Mean difference of measures for tasks with labels compared to baseline, grouped by placement method. Bold p-values indicate that the measured difference from the baseline is significant.\newline
%     $\overline{B}_{x}$ = mean of measures with baseline labels \newline
%     $\overline{L}_{x}$ = mean of measures with color, texture or shape labels
% }

  
%   \label{table:mean_diff}
%   \begin{tabular}{r l l l l l}
%     \toprule
%     %&&Number of&Number of&&\\
%      & & \multicolumn{4}{c}{\textbf{Placement}} \\
%      \cmidrule(r){3-6}
%       &&\multicolumn{2}{c}{\textbf{Dim. reduction}}& \multicolumn{2}{c}{\textbf{Random}} \\
%       \textbf{Measure}&\textbf{Label}& \textbf{$\overline{B}_{DR} -\overline{L}_{DR}$} &\textbf{p-value}&\textbf{$\overline{B}_{R} -\overline{L}_R$}  &\textbf{p-value}\\
%     \midrule
%     Time (s) &&&&\\
%     & Shape   & 1.59 & 0.18 &-1.58 & 0.26\\
%     & Color   & 0.76 & 1.0 &-0.9  & 1.0\\
%     & Texture & 0.73 & 0.96 &-2.91 & \textbf{0.03} \\
%     Hovered&&&&\\
%     samples& Shape & 6.9 & \textbf{4e-07} &6.0 & \textbf{0.002}\\
%     & Color & 1.4 & 0.89  & 1.9 & 0.52 \\
%     & Texture & 1.5 & 0.33  & 2.7 & 0.13 \\
%     Total distance &&&&\\
%     (pixels) & Shape & 493 & \textbf{0.04} & -30 & 1.0 \\
%     & Color & 41 & 1.0  & -493 & 0.20 \\
%     & Texture & 120 & 0.94  & -307 & 0.61 \\
    
%     \bottomrule
% \end{tabular}
% \end{table*}


%put actual p-values (more information) opens up for discussion about sample size

%maybe talk about sample size needed for difference to become significant. %post-hoc power analysis 

\subsubsection{Effect of iteration}
\label{results:b:iteration}
Given that participants complete the study multiple times, we are curious whether they improve at the different tasks over time.

Overall, we do not see a significant effect of iteration on measures. However, in baseline tasks with DR placement, there is a significant difference between completion times (p=0.0078) and mouse speed (p=0.00020) when comparing between the first and subsequent iterations. We hypothesize that participants were still becoming accustomed to using the interface during this first task in the study. 
There are no significant differences between iterations for tasks with random placement. When inspecting the data visually, there is also a noticeable downward trend for tasks with labels and DR-based placement times over iterations, but the differences do not pass significance testing. 

\subsubsection{Questionnaire results}
\label{results:b:questionnaire}

The responses to many questions did not show significant differences between label types. This section highlights the most interesting responses. A full list of the questions can be found in the supplementary materials (Online Resource 1, section 5).

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{images/consistency_likert.eps}
  \caption{Responses to the questions about the perceived consistency of the labelling and placement methods }
  \label{fig:consistency}
\end{figure}

Figure \ref{fig:consistency} shows Likert plots of responses to questions about the perceived consistency of the placement of samples and the labelling methods in labelled tasks with DR placement. When rating label consistency, participants are quite evenly divided on texture labels, and lean towards color being more consistent. In the case of shapes, none rated their consistency below 3. When asked to rate whether similar sounds were located closer together, more participants responded with lower ratings after tasks with shape labels (p=0.032).

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{images/help_likert.eps}
  \caption{Responses to the questions about the perceived helpfulness of the labels and the sample placement}
  \label{fig:coordinates_help}
\end{figure}

Figure \ref{fig:coordinates_help} shows Likert plots of ratings of the perceived helpfulness of the placement of the samples during labeled tasks with DR placement. After tasks with color and texture labels, ratings skew towards the placement being helpful, but after tasks with shape labels they rate the placement as being less helpful (p= 0.04). This indicates that participants were perhaps paying less attention to the placement when shape labels were provided. 
Participants are quite evenly divided between positive and negative responses when rating the helpfulness of all of the label types.
% Use test for different means within same population
% Compare proportion that answered 3 or more (because medians are the same) 


\subsection{Online study}
\label{results:c}
Participants performed this study on their own computers, and were less experienced than participants in the previous study. While we used the same minimum experience criteria for both studies, 10 out of the 15 participants in the controlled environment study had at least 10 years of experience while 13 out of the 14 participants in this study had between 2 and 5 years of experience. 

\subsubsection{Effect of placement methods}
\label{results:c:place}

% Table \ref{table:mean_label_groups_class} shows mean measures grouped by placement and labeling methods and 

Figure \ref{fig:group_means_class} shows mean measures grouped by placement and labeling method with 95\% confidence intervals. The only significant difference between placement methods is found in tasks with texture labels, where participants moved their cursor over $\sim$1200 more pixels searching for the target sound when positions were randomized. The exact means and p-values are provided in the supplementary materials (Online Resource 1, section 3, table S1).

% %Todo make sure these are actually correct
% \begin{table}[h]
%   \caption{Means of measures grouped by placement and labeling methods. Bold p-values show when the measured difference between placement methods is significant.}
%   \label{table:mean_label_groups_class}
%   \begin{tabular}{l l l l l}
%     \toprule
%     %&&Number of&Number of&&\\
%      \textbf{Measure}& \textbf{Label}& \multicolumn{2}{c}{\textbf{Placement}} & \textbf{p-value}\\
%      \cmidrule(r){3-4}
%       &&\textbf{DR} &\textbf{Random} & \\
%     \midrule
%     Time &&&&\\
%     & Baseline & 7.9 & 9.0  & 0.34 \\
%     & Shape & 8.0 & 9.4 & 0.59\\
%     & Color & 10.5 & 8.2 & 0.20\\
%     & Texture & 9.0 & 12.0 & 0.09\\
    
%     Hovered&&&&\\
%     samples& Baseline & 15.0& 16.5 & 0.75\\
%     & Shape & 14.0 & 13.4 & 0.99\\
%     & Color & 16.4 & 11.5 & 0.15\\
%     & Texture & 16.2 & 19.2 &0.69\\

%     Distance &&&&\\
%     & Baseline & 2785 & 3024 & 0.68\\
%     & Shape & 2714 & 3156 & 0.67 \\
%     & Color & 3118 & 2752 & 0.75\\
%     & Texture & 2935 & 4160 & \textbf{0.026}\\
%     \bottomrule
% \end{tabular}
% \end{table}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{images/summer_class_double.eps}
  \caption{Means of measures grouped by label type and positioning. 95\% confidence intervals shown as error bars.}
    \label{fig:group_means_class}
\end{figure}

\subsubsection{Effect of labeling methods}
\label{results:c:label}

Table \ref{table:mean_diff_online} shows the differences between labelled tasks and the baseline. There are two significant differences in completion times; on average, tasks with color labels and DR placement took 2.5 seconds longer than the baseline, while tasks with texture labels and random placement took 3 seconds longer than the baseline. 
5 less samples were visited on average in tasks with color labels and random placement compared to the baseline. Finally, when comparing mouse travel distance, in tasks with texture labels and random placement, participants covered ~1100 more pixels than the baseline.



\begin{table}[h]
  \caption{Mean difference of measures compared to baseline, grouped by placement method. Positive values indicate an improvement. Bold p-values indicate that the measured difference is significant.\newline
      $\overline{B}$ = mean of measures with baseline labels \newline
    $\overline{L}$ = mean of measures with color, texture or shape labels
    \newline DR = placement by dimensionality reduction.
}
  \label{table:mean_diff_online}
  \begin{tabular}{l l l l l l}
    \toprule
    %&&Number of&Number of&&\\
     & & \multicolumn{4}{c}{\textbf{Placement}} \\
     \cmidrule(r){3-6}
      &&\multicolumn{2}{c}{\textbf{DR}}& \multicolumn{2}{c}{\textbf{Random}} \\
      \textbf{Measure}&\textbf{Label}& \textbf{$\overline{B} -\overline{L}$} &\textbf{\textit{p-val.}}&\textbf{$\overline{B} -\overline{L}$}  &\textbf{\textit{p-val.}}\\    \midrule
    Time &&&&\\
    & Shape   & -0.1 & 1.0 & -0.4 & 0.97 \\
    & Color   & -2.5 & \textbf{0.05} & 0.8  & 0.82 \\
    & Texture & -1.1 & 0.56 & -3.0 &  \textbf{0.05}\\
    
    Hovered&&&&\\  
    samples& Shape & 1.0 & 0.96 & 3.1 & 0.50 \\
    & Color & -1.4 & 0.92 & 5.0 & \textbf{0.05} \\
    & Texture & -1.3 & 0.93  & -2.7 & 0.71\\
    
    Distance &&&&\\
    & Shape & 71 & 0.99  & -131& 0.98 \\
    & Color & -333 & 0.72 & 272 & 0.82 \\
    & Texture & -150 & 0.95  & -1136 & \textbf{0.02} \\
    \bottomrule
\end{tabular}
\end{table}



% \begin{table*}[h]
%   \caption{Mean difference of measures compared to baseline, grouped by placement method. Positive values indicate an improvement. Bold p-values indicate that the measured difference is significant.\newline
%       $\overline{B}_{x}$ = mean of measures with baseline labels \newline
%     $\overline{L}_{x}$ = mean of measures with color, texture or shape labels}
%   \label{table:mean_diff_online}
%   \begin{tabular}{r l l l l l}
%     \toprule
%     %&&Number of&Number of&&\\
%      & & \multicolumn{4}{c}{\textbf{Placement}} \\
%      \cmidrule(r){3-6}
%       &&\multicolumn{2}{c}{\textbf{Dim. reduction}}& \multicolumn{2}{c}{\textbf{Random}} \\
%       \textbf{Measure}&\textbf{Label}& \textbf{$\overline{B}_{DR} -\overline{L}_{DR}$} &\textbf{p-value}&\textbf{$\overline{B}_{R} -\overline{L}_R$}  &\textbf{p-value}\\    \midrule
%     Time &&&&\\
%     & Shape   & -0.1 & 1.0 & -0.4 & 0.97 \\
%     & Color   & -2.5 & \textbf{0.05} & 0.8  & 0.82 \\
%     & Texture & -1.1 & 0.56 & -3.0 &  \textbf{0.05}\\
    
%     Hovered samples &&&&\\  
%     & Shape & 1.0 & 0.96 & 3.08 & 0.50 \\
%     & Color & -1.4 & 0.92 & 5.0 & \textbf{0.05} \\
%     & Texture & -1.3 & 0.93  & -2.7 & 0.71\\
    
%     Total distance &&&&\\
%     & Shape & 71 & 0.99  & -131& 0.98 \\
%     & Color & -333 & 0.72 & 272 & 0.82 \\
%     & Texture & -150 & 0.95  & -1136 & \textbf{0.02} \\
%     \bottomrule
% \end{tabular}
% \end{table*}

==> sections/study_descriptions.tex <==

\section{Studies}
\label{results}

We conducted our study with 3 different groups of participants. The preliminary study did not lead to significant conclusions, prompting us to perform a study in a controlled environment with specifically qualified participants. Based on feedback from this second study, we decided to change the manner in which color labels were generated. We conducted a third iteration of the study with two objectives in mind : testing the new color labels and comparing the quality of results obtained in controlled and uncontrolled environments.

\subsection{Winter 2019: initial study}
\label{results:initial}
The precursor to this article \citep{richan_study_2019} summarized the results from a group of 28 computer engineering students. Students completed the study as part of coursework in a class on human perception. Students performed the study on their own computers, but were instructed to use a computer mouse and earphones. Based on those results, we concluded that it would be worthwhile to recruit a group of participants with a minimum of 2 years musical experience to perform the study in a controlled environment. We also realized the need for the baseline task with random placement, which was originally not part of the study. We only compared completion times in this study, and decided to record more data points in follow-up studies. 

\subsection{Summer 2019: qualified participants in a controlled environment}
\label{results:onsite}
15 participants were recruited from the music and engineering faculties of the University of Sherbrooke. They were required to have at least two years of recent experience working with sound which would adequately qualify them for the task of differentiating sounds by timbre alone. Participants completed the study in a secluded area on tablet-style laptops with a connected mouse and keyboard. The testing stations were equipped with Sennheiser HD 280 Pro headphones, connected via a Rega EAR amplifier and a Roland UA-1G USB interface.

Participants completed three passes of the study, with each iteration testing a different labelling method. Given that there are 3 types of labels, there are 6 permutations of the order they could be tested. These permutations were distributed between participants as evenly as possible.

% The progression through the study and the number of tasks performed for each task type are summarized in table \ref{table:progression}. We decided to not include $B_R$ in the first iteration as we thought it would take much longer than other task sets and might discourage participants to start with a more difficult task. 


% \begin{table*}[h]
%   \caption{Study B steps}
%   \label{table:progression}
%   \begin{tabular}{l l l l l l l l l }
%     \toprule
%     %&&Number of&Number of&&\\
%   \textbf{1st iteration tasks} & $Q_0$ &Practice &$B_C$&$L_C$&$Q_1$&$L_R$&$Q_2$ \\
%     Familiarization tasks& & 1& 6&6&&0&\\
%     Evaluation tasks& & 0& 6&8&&10&&\\
    
%     \midrule
%     \textbf{2nd, 3rd iteration tasks} && $B_R$ &$B_C$&$L_C$&$Q_1$&$L_R$&$Q_2$\\
%     Familiarization tasks&& 0& 6&6&&0&\\
%     Evaluation tasks&& 6& 6&8&&10&\\
%     \bottomrule
% \end{tabular}
% \begin{description}$Q_0$, $Q_1$ and $Q_2$ are short questionnaires.
% \end{description}
% \end{table*}

\subsection{Summer 2019: new color labels and online participants}
A second group of participants, recruited in the same manner as the initial study, performed the study on their personal computers. For our analysis, we used results from 14 participants who reported more than two years musical experience and having completed the study in good listening conditions. 

\color{red} 
We changed the way in which color labels were generated to better correspond other work in the field, particularly \cite{Grill2012VisualizationOP} and \citep{adeli_audiovisual_2014}. Our new method uses direct mapping from timbral descriptors to the hue and saturation of the circular labels. 
The spectral centroid (measuring timbral brightness) is mapped to a gradient from blue to red and spectral flatness (measuring tonality) is then mapped to the color's saturation. 
\color{black}
Shape and texture labels remain unchanged.

%Each student completed the study twice, but many did not correctly report whether it was their first or second time.
% The participants progressed through task sets in a manner similar to the previous study see table \ref{table:student_progression}.

% Based on our conclusions from the initial study, 

% \begin{table*}[h]
%   \caption{Study C steps}
%   \label{table:student_progression}
%   \begin{tabular}{l l l l l l l l l }
%     \toprule
%      & $Q_0$ &Practice &$B_R$&$B_C$&$L_C$&$ Q_1$&$L_R$&$Q_2$ \\
%     Familiarization tasks& & 1& 6&6&6&&0&\\
%     Evaluation tasks& & 0& 6&8&6&&10&&
%     \bottomrule
% \end{tabular}
% \begin{description}
% \end{description}
% \end{table*}
 


% todo : actual equations?

==> sections/study_design.tex <==

\section{Study design}
\label{design}
The goal of our study is to determine whether and to what extent different types of labels (shape, color, and texture) help in the task of searching for a specific sample in a starfield display. The secondary objective is to evaluate the effectiveness of our dimensionality reduction based placement approach (section \ref{design:coords}). We designed a known-item search task that would allow us to test different combinations of labelling and placement methods. In order to obtain a baseline for comparison, we create baseline variants for labels and placement. The label baseline uses grey circles to represent each sample and the placement baseline assigns random coordinates to each sample.

\subsection{Task design and interaction}
\label{design:task}

The task interface (with baseline labels) is shown in figure \ref{fig:interface}. In each task, 30 sounds are picked at random from a dataset and one is designated as the target sound the participant must find. Individual sound samples are displayed as circular shapes arranged on a light grey canvas. Samples are played by mousing over the corresponding element. Pressing the space bar plays the target sound and clicking on the correct element completes the task. Before each task, the participant must place their cursor in a corner of the canvas. This corner rotates clockwise around the canvas between tasks in order to vary the starting point. 

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{images/interface.png}
  \caption{The task interface used in the study. \textit{Left} : The intermediary screen shown before each task. \textit{Right} : An example of a baseline task. Red outlines indicate an incorrectly clicked sound while a green outline highlights the current playing sound.}
\label{fig:interface}
\end{figure}


\subsection{Sets of tasks to introduce and evaluate timbre visualisation methods}
\label{design:task_sets}

Participants progress through the study by completing sets of tasks that introduce and evaluate the placement method and the visual labels. They first complete a practice task, which uses baseline labels and random placement, that they repeat until they are certain they understand how the interface works. They then complete a set of tasks with baseline labels and random placement. This represents the worst-case scenario, where no relevant information is being visualised. 

The rest of the study progresses by alternating between familiarization and evaluation tasks. During familiarization tasks, participants are encouraged to take their time and explore the set of samples while searching for the target sound. During evaluation tasks, participants are instructed to find the target sound as quickly as possible. We first introduce the dimensionality reduction (DR) based placement method with baseline labels. We then introduce a visual labelling method (color, shape or texture) with a set of tasks that uses the DR placement. Finally, we test the effectiveness of the labels on their own in a final set of tasks with the same labelling method and random placement. Before each set of tasks, participants read some brief instructions, which can be found in the supplementary materials of the paper (Online Resource 1, section 6).

The two placement methods (random and DR), and four label types (baseline, color, shape and texture) combine to form 8 different testing conditions. 
Participants also complete three survey-style questionnaires during the study referred to as $Q_0$, $Q_1$ and $Q_2$. In $Q_0$, participants provide basic demographic information (e.g. age, listening conditions, years of experience). In $Q_1$ and $Q_2$, participants are asked to rate the extent to which they used different search strategies for finding the target sound. They are also asked to rate whether the positioning or labeling of the sounds helped them in their search and how difficult they found the task overall. See the supplementary materials (Online Resource 1, section 5) for the full list of questions.

We designed the study to introduce and evaluate each of three types of labels separately. Table \ref{table:basic_progression} summarises how a participant would progress through the entire study. For each set of task conditions, the same task will be repeated 5-10 times (depending on the task) with new samples each time. We designed the study to take approximately 30 minutes to complete. 



% Samples are placed according to precalculated coordinates (section \ref{design:coords}) or random placement. Combining these placement methods with the labelling methods produces eight distinct task sets, shown in table \ref{table:tasks}. From this point on, we will use the symbols in the table to refer to the different test conditions. We use the symbols $L_C$ and $L_R$ to refer to tasks with labels with coordinate-based or random placement respectively. There is also an initial practise task, 

% We designed our study to compare three types of visual labels in a known-item search task.

% For each task set aside from $L_R$, and $B_R$ there is a an initial familiarization set of tasks, followed by an evaluation set of tasks. Before each set of tasks participants read some brief instructions.  In $B_C$ familiarization tasks, they are instructed to investigate whether nearby samples produce similar sounds. In $L_C$ familiarization tasks, instructions are to explore whether visually similar samples produce similar sounds. In $L_R$ tasks, participants are informed that positional information will no longer be of use and that they should try to use the labels to guide their search.



% \begin{table*}[h]
%   \caption{Acronyms used to refer to combinations of task conditions. We use $L_X$ to refer to all three label types.}
%   \label{table:tasks}
%   \begin{tabular}{l l l l l l }
%     \toprule
%     \textbf{} & \textbf{Baseline} &\textbf{Color}&\textbf{Shape} &\textbf{Texture} & \textbf{[Color, Shape, Texture] } \\
%     \midrule
%     \textbf{Dim. reduction} & $B_{DR}$ & $C_{DR}$& $S_{DR}$ &$T_{DR}$ & L_{DR}\\
%     \textbf{Random}  & $B_R$ &$C_R$ &$S_R$ &$T_R$ & $L_R$ \\    
%     \bottomrule
% \end{tabular}
% \end{table*}

\begin{table}[h]
  \caption{ Series of tasks that participants complete while progressing through the study.
  \newline $P=$ Practice, $B_x$ = Baseline labels. $L_x$ = Color, shape or texture labels, $x_{DR}$=  Task with dimensionality reduction placement, $x_{R}$= Task with random placement
  }
  \label{table:basic_progression}
  \begin{tabular}{l l l l l l l l l }
    \toprule
    \textbf{Order} &1&2 &3&4&5&6 &7 &8  \\
    \midrule
    \textbf{Task type} &$Q_0$ &$P$ &$B_R$&$B_{DR}$&$L_{DR}$&$ Q_1$&$L_{R}$&$Q_2$ \\
    \bottomrule
\end{tabular}

\end{table}


\subsection{NSynth dataset and timbre feature extraction for sample placement and label generation}
\label{design:dataset}

We use musical samples from the NSynth dataset \citep{engel_neural_2017}, which consists of over 300,000 four-second samples produced by virtual instruments in commercial sample libraries. We are interested in differentiating timbre, so we use a subset of $\sim$800 samples with the same pitch and velocity. We use samples at midi note 64, which corresponds to musical note E4. 

For each sample, we use a cochlear filterbank\footnote{Available for download from \url{https://github.com/NECOTIS/ERBlet-Cochlear-Filterbank}} \citep{adeli_flexible_2016} to extract three profiles related to the perception of timbre: a spectral envelope, a roughness envelope (which measures perceived auditory roughness over time) and a temporal amplitude envelope. These timbre features are used both to determine sample placement as well as generate visual labels.

\subsection{Sample placement through dimensionality reduction} 
\label{design:coords}
We obtain two-dimensional coordinates for the musical samples by performing dimensionality reduction (DR) on the extracted features. We first use PCA to reduce each profile to a shorter feature vector, then apply UMAP \citep{mcinnes2018umap-software} on the concatenated vectors to produce a 2D arrangement of the samples that represents the distances between their high-dimensional timbre features. Recent related work \citep{frisson_audiometro:_2014,font_corbera_freesound_2017} has used t-SNE \citep{van_der_maaten_visualizing_2008} for dimensionality reduction, however, we find that UMAP obtains comparable results in significantly less computation time. %(on the cpu) new cuML CUDA tsne is much faster

During testing, samples would occasionally overlap in the interface. To remedy this, before displaying each task, we run a brief physical simulation by placing virtual springs between samples causing them to push away from each other if they are overlapping. 


\begin{figure*}[h]
  \centering
  \includegraphics[width=\textwidth]{images/label_types_zoom.png}
  \caption{The three types of visual labels for the same set of randomly selected sound samples. From left to right: shape, color, texture.}
  \label{fig:methods}
  %\begin{description}
   % From left to right: Shape, color, Texture.
  %\end{description}
%   Boxes highlight samples presented in figure \ref{fig:samples}}
\end{figure*}
\subsection{Visual label generation}
\label{design:labels}

Research on human visual perception has revealed that separate pathways are used to process shape, color and texture \citep{cant_independent_2008}. While this indicates that shape, color and texture could be used to distinguish between visual samples in a complementary fashion, this is not always the case. Different types of visual information can also interfere with each other \citep{callaghan_interference_1989}, so our study will test each of these pathways separately. 
%This is why we do not combine visualisation methods in our study.

%could cut first sentences 

% Many information visualisation paradigms use a small number of perceptually distinct colors and symbol-shapes (squares, triangles, crosses, etc.) to differentiate between categories. These types of representations require some form of pre-existing or extracted categorical metadata to be associated with the file. 
In our study, we are interested in differentiating timbre, which is often represented by continuous features describing some aspect of the spectral or temporal characteristics of the sound. We generate labels that vary continuously by using mappings from timbral features to visual parameters. Figure \ref{fig:methods} shows how the same set of samples would appear for each type of visual label. Labels could be of varying sizes, but for our studies, sample labels were 64 square pixels.

\subsubsection{Shape}
\label{design:labels:shape}

We use the temporal envelope (section \ref{design:dataset}) to generate our shapes because it visualises the attack time and low-frequency amplitude modulations in the signal, which are important timbral descriptors \citep{mcadams_perceptual_1995}.
We produce a unique shape for each sound by mapping the amplitude of the temporal envelope to the contour of a circular shape. We downsample the envelope to obtain a 20ms temporal resolution. This produces 200 distinct points for our 4 second samples. The radius of each point on a half-circle is described by equation \ref{eq:circle}.
\begin{equation}\label{eq:circle} 
R\left( {\theta } \right) = envelope[i],\,\,\,\theta  = \frac{i \cdot \pi }{{200}},\,\,\,i \in \left\{ {0,200} \right\}
\end{equation}

This half-circular shape is then rotated and mirrored along the x-axis to produce a symmetrical shape. The topmost point of the shape represents the amplitude of the envelope at the beginning of the sound and the bottom-most point the amplitude at the end of the sound.
\color{red}
This method is comparable to \citep{heise_aurally_2009}, with the main difference being that our approach produces symmetrical shapes, which are known to be easier to perceive and remember \citep{ward_multivariate_2008}.

\color{black}
%Maybe mention that symmetrical shapes are better but have to find paper)


\subsubsection{Color}
\label{design:labels:color}
For color, we use a simpler approach based on the coordinates of the samples in the reduced 2D space. The center of the spatial distribution of the entire set of samples is calculated and each sample is assigned a color based on its position relative to the center. The hue is determined by its angle relative to the center point and the saturation is determined by its distance to the center point. 
\color{red}
This can be imagined as laying a color wheel over the entire sample distribution and picking a color for each sample based on their location within it. Each sample's color reinforces the spatial information which is based on timbral similarity.
\color{black}
% TODO : equations

\subsubsection{Texture}
\label{design:labels:texture}
We developed a software tool to generate textural labels for the samples.
 \color{red}

% Our method for textures is quite different from traditional visualisation theory approaches 
% Texture synthesis is an ongoing challenge in machine learning and image processing. 
% Computer vision research has produced effective tools for synthesizing textures from reference images [markov random, self tuning]. 

% The method we chose strikes a balance between image quality, speed and GPU load.
% Non-neural network approaches are probably faster, and better, but aren't as cool-sounding.
% Also the network approach gives us the possibility of stylising

We use  Li et al.'s method for "universal" style transfer  \citep{li_universal_2017} to synthesize textures based on reference images. The method uses a pre-trained encoder-decoder deep convolutional network (provided by \citep{li_universal_2017}). The encoder is an image classification network \citep{simonyan_very_2015}, while the decoder is pre-trained to reconstruct images from the activation patterns of the encoder. Noise is fed into the encoder network and the activation pattern is transformed to resemble that of a reference texture. The decoder can then produce a new image with textural properties that greatly resemble the original image. This method can be used to interpolate between textures by using a weighted sum of their activation patterns.
\color{black}



Eight medioids \citep{jin_k-medoids_2010} are found in the timbre space and each one is manually assigned a texture from the normalized Brodatz texture database \citep{abdelmounaime_new_2013}. We use black and white texture images in order to differentiate from the color method. We choose visually distinct textures for each medioid, and attempt to relate properties of the sounds to textural characteristics (e.g. a rapidly varying synth note is labeled with a chaotic rootlike texture, while a percussive mallet note is labeled with a texture of pebbles in an attempt to evoke the hardness of the material being struck). Textures for all the other sounds in the dataset are then produced by the texture synthesis method by interpolating between these textures based on their proximity to the medioids. 
\color{red}
Through this process, samples are assigned textural images whose visual properties vary in tandem with their timbral difference.

\color{black}


\subsection{Technologies used}
\label{design:technologies}
We use JATOS \citep{lange_just_2015} to build and host our study on a webserver, which allows us to easily distribute the study to participants using a web link. JATOS studies are executed in the browser so no installation is required for the participants. 
The filterbank, dimensionality reduction and label generation are implemented in Python, and the resulting information is stored in a dictionary JSON file on the webserver that is loaded by the web application. Pre-calculated shape and color information are stored as arrays in the dictionary. Each sample entry also points to a pre-generated JPEG texture file that is stored on the webserver. We use \textit{jsPsych} \citep{de_leeuw_jspsych:_2015} and \textit{p5.js} \citep{lauren_mccarthy_p5.js_nodate} to build the interactive components of the study and \textit{toxiclibs.js} \citep{kyle_phillips_toxiclibs.js_nodate} for the spring physics simulation. 

\subsection{Collected data }
\label{measures}

The measures we use to evaluate and compare labelling methods are summarized in table \ref{table:measure}. We collect several other data points from tasks, including the entire cursor trajectory, cursor speed, the number of misidentified samples and the number of times the participant listened to the target sound. The anonymised data collected in our studies will be available in the supplementary materials repository \citep{richan_timbre_2019}.
\begin{table}[ht]
  \caption{Recorded measures used to evaluate task performance}
  \label{table:measure}
  \begin{tabular}{l l l}
    \toprule
    %&&Number of&Number of&&\\
     \textbf{Measure}& \textbf{Description} &\textbf{Units} \\
    \midrule
    Time & Time taken to complete  &Seconds\\
    & the task&\\
    Hovered samples & Number of samples the & Count\\
    & cursor encountered & \\
%    Mouse speed & Average sped of the mouse cursor& Pixels/second\\
    Distance & Total distance the mouse & Pixels\\
     & cursor travelled &\\
    \bottomrule

\end{tabular}
\end{table}

In summary, we designed this study to evaluate the effect of both visual labels and placement while searching for musical samples in a media browser using technologies allowing for simple and easy distribution to participants. The studies we conducted using this design were approved by the \textit{Comité d’éthique de la recherche - Lettres et sciences humaines} of the University of Sherbrooke (ethical certificate number 
2018-1795).
 



